Toward End-to-End MLOps Tools Map: A Preliminary Study based on a Multivocal Literature Review

MLOps tools enable continuous development of machine learning, following the DevOps process. Different MLOps tools have been presented on the market, however, such a number of tools often create confusion on the most appropriate tool to be used in each DevOps phase. To overcome this issue, we conducted a multivocal literature review mapping 84 MLOps tools identified from 254 Primary Studies, on the DevOps phases, highlighting their purpose, and possible incompatibilities. The result of this work will be helpful to both practitioners and researchers, as a starting point for future investigations on MLOps tools, pipelines, and processes.

==> Section/Study_backup.tex <==
\section{Study Design (2 pages)}
\label{Study}

The goal of our study is to associate all the tools supporting MLOps with MLOPs phases with the purpose of outlining a fully-supported MLOps pipeline. The perspective is of both researchers and practitioners. The former could build on top of our result to build new knowledge and propose new methods. The latter could benefit from our results to improve their MLOps development procedures.

To this aim, we first need to gather all the MLOps tools available in the literature and associate them to all MLOps phases they support. This lead us to the definition of our first research question:

\begin{center}	
	\begin{rqbox}
		\textbf{RQ$_1$.} \emph{To what extent the different phases of MLOps are supported by tools?}
	\end{rqbox}	
\end{center}

After having retrieved all the information about the tools and the phases they support, we aim to explore all the possible combinations of them with the purpose of building a fully supported and automated MLOps pipeline:

\begin{center}	
	\begin{rqbox}
		\textbf{RQ$_2$.} \emph{What are the possible combinations of tools to support a pipeline in MLOps?}
	\end{rqbox}	
\end{center}

In the following, we provide details on the methods we adopted to address both research questions.

\subsection{RQ$_1$ - Mapping MLOps tools on MLOps pipeline}

Our first research question's goal is to map the available MLOps tools on the MLOps pipeline. This will allow us to understand to what extent the MLOps pipeline is actually supported and what are the steps that require additional support.

To fulfill this goal, we started from a recent Multivocal Literature Review (MLR) by Recupito et al.~\cite{Recupito2022} that reports detailed information about the MLOps tools available so far. More details about this study are reported in Section~\ref{Background}.

This led us to collect a first set of 13 MLOps tools.

However, while this study only focuses on MLOps-specific tools, it is worth considering that there could exist other tools (e.g., tools supporting DevOps) that also provide support for MLOps pipelines.

For this reason, we decided to complement Recupito et al.'s MLR with another step-by-step MLR with the aim of collecting all these additional pieces of information.

We followed the three steps defined by Kitchenham et al.~\cite{kitchenham2004procedures}: first we defined a search string, then we applied it to the search engines of our choice, and finally we filtered and extracted the studies basing on our defined inclusion and exclusion criteria.

For each step of the MLOps pipeline (\todo[inline]{Add a reference to the MLOps figure that will be added in the Background}) we performed a search of both white and grey sources by running the following search query:

\begin{center}
   \todo[inline]{Here to add the search query}
\end{center}

As for the white literature, we performed our search on Google Scholar, while we relied on Google and \textcolor{red}{XXX} for the grey literature.

We checked each extracted source to ensure it fitted with our goal, according to the following exclusion and inclusion criteria:

\smallskip
\noindent
\textbf{Inclusion Criteria:} 
\begin{enumerate}
    \item \textcolor{red}{IC1}.
    \item \textcolor{red}{IC2}.
    \item \textcolor{red}{IC3}.
\end{enumerate}
\smallskip
\noindent
\textbf{Exclusion Criteria:}
 \begin{enumerate}
    \item \textcolor{red}{EC1}.
    \item \textcolor{red}{EC2}.
    \item \textcolor{red}{EC3}.
\end{enumerate}

Once extracted a final set of tools from the described process, we merged them with those reported by Recupito et al.~\cite{Recupito2022} inorder to have a finalsetof toolssupporting MLOps to further analyze.

 \textcolor{red}{Two of the authors performed a manual inspection of the documentation with the aim of associating each tool with all the supported steps of the MLOps pipeline. In case of conflicts, a third author performed an additional check. We measured the agreement.}
 
\todo[inline]{To add a figure reporting the entire process. Euromicro's tools + the step-by-step MLR.}


%Based on tools documentation, we associate each tool with the corresponding phases

\subsection{RQ$_2$ - Combining tools for a fully-supported pipeline}

%First we analyzed all the couples of potential combinations (tools that cover complementary phases)

%For each couple we checked requirements in the documentation (e.g., only AWS)

%Finally, we simulated and executed the combination.
